STRIDE: When to Speak Meets Sequence Denoising for Streaming Video Understanding

Recent progress in video large language models (Video-LLMs) has enabled strong offline reasoning over long and complex videos. However, real-world deployments increasingly require streaming perception and proactive interaction, where video frames arrive online and the system must decide not only what to respond, but also when to respond. In this work, we revisit proactive activation in streaming video as a structured sequence modeling problem, motivated by the observation that temporal transitions in streaming video naturally form span-structured activation patterns. To capture this span-level structure, we model activation signals jointly over a sliding temporal window and update them iteratively as new frames arrive. We propose STRIDE (Structured Temporal Refinement with Iterative DEnoising), which employs a lightweight masked diffusion module at the activation interface to jointly predict and progressively refine activation signals across the window. Extensive experiments on diverse streaming benchmarks and downstream models demonstrate that STRIDE shows more reliable and temporally coherent proactive responses, significantly improving when-to-speak decision quality in online streaming scenarios.

==> assets/dvc_LfSYF1N5i_Q/question.tex <==
Dense captioning: "making tomato soup"

==> assets/dvc_LfSYF1N5i_Q/response.tex <==
GT[0]: [44.0,63.0]s IoU=0.79 ~~ GT[1]: [63.0,93.0]s IoU=0.52 ~~ GT[2]: [95.0,126.0]s IoU=0.33 ~~ GT[3]: [143.0,194.0]s IoU=0.69 ~~ GT[4]: [198.0,216.0]s IoU=0.82

==> assets/dvc_LfSYF1N5i_Q/time1.tex <==
0s

==> assets/dvc_LfSYF1N5i_Q/time10.tex <==
83s

==> assets/dvc_LfSYF1N5i_Q/time11.tex <==
91s

==> assets/dvc_LfSYF1N5i_Q/time12.tex <==
100s

==> assets/dvc_LfSYF1N5i_Q/time13.tex <==
103s

==> assets/dvc_LfSYF1N5i_Q/time14.tex <==
114s

==> assets/dvc_LfSYF1N5i_Q/time15.tex <==
116s

==> assets/dvc_LfSYF1N5i_Q/time16.tex <==
126s

==> assets/dvc_LfSYF1N5i_Q/time17.tex <==
133s

==> assets/dvc_LfSYF1N5i_Q/time18.tex <==
143s

==> assets/dvc_LfSYF1N5i_Q/time19.tex <==
149s

==> assets/dvc_LfSYF1N5i_Q/time2.tex <==
17s

==> assets/dvc_LfSYF1N5i_Q/time20.tex <==
153s

==> assets/dvc_LfSYF1N5i_Q/time21.tex <==
164s

==> assets/dvc_LfSYF1N5i_Q/time22.tex <==
166s

==> assets/dvc_LfSYF1N5i_Q/time23.tex <==
174s

==> assets/dvc_LfSYF1N5i_Q/time24.tex <==
183s

==> assets/dvc_LfSYF1N5i_Q/time25.tex <==
185s

==> assets/dvc_LfSYF1N5i_Q/time26.tex <==
195s

==> assets/dvc_LfSYF1N5i_Q/time27.tex <==
199s

==> assets/dvc_LfSYF1N5i_Q/time28.tex <==
206s

==> assets/dvc_LfSYF1N5i_Q/time29.tex <==
216s

==> assets/dvc_LfSYF1N5i_Q/time3.tex <==
33s

==> assets/dvc_LfSYF1N5i_Q/time30.tex <==
224s

==> assets/dvc_LfSYF1N5i_Q/time31.tex <==
232s

==> assets/dvc_LfSYF1N5i_Q/time32.tex <==
248s

==> assets/dvc_LfSYF1N5i_Q/time4.tex <==
44s

==> assets/dvc_LfSYF1N5i_Q/time5.tex <==
50s

==> assets/dvc_LfSYF1N5i_Q/time6.tex <==
56s

==> assets/dvc_LfSYF1N5i_Q/time7.tex <==
66s

==> assets/dvc_LfSYF1N5i_Q/time8.tex <==
67s

==> assets/dvc_LfSYF1N5i_Q/time9.tex <==
79s

==> assets/epm_8a89601b/question.tex <==
Find event answering: "How many pots did I see on the gas cooker?"

==> assets/epm_8a89601b/response.tex <==
GT[0]: [32.9,39.4]s IoU=0.77

==> assets/epm_8a89601b/time1.tex <==
0s

==> assets/epm_8a89601b/time10.tex <==
39s

==> assets/epm_8a89601b/time11.tex <==
48s

==> assets/epm_8a89601b/time12.tex <==
60s

==> assets/epm_8a89601b/time13.tex <==
72s

==> assets/epm_8a89601b/time14.tex <==
84s

==> assets/epm_8a89601b/time15.tex <==
96s

==> assets/epm_8a89601b/time16.tex <==
108s

==> assets/epm_8a89601b/time17.tex <==
120s

==> assets/epm_8a89601b/time18.tex <==
132s

==> assets/epm_8a89601b/time19.tex <==
144s

==> assets/epm_8a89601b/time2.tex <==
12s

==> assets/epm_8a89601b/time20.tex <==
156s

==> assets/epm_8a89601b/time21.tex <==
168s

==> assets/epm_8a89601b/time22.tex <==
180s

==> assets/epm_8a89601b/time23.tex <==
192s

==> assets/epm_8a89601b/time24.tex <==
204s

==> assets/epm_8a89601b/time25.tex <==
216s

==> assets/epm_8a89601b/time26.tex <==
228s

==> assets/epm_8a89601b/time27.tex <==
240s

==> assets/epm_8a89601b/time28.tex <==
252s

==> assets/epm_8a89601b/time29.tex <==
264s

==> assets/epm_8a89601b/time3.tex <==
24s

==> assets/epm_8a89601b/time30.tex <==
276s

==> assets/epm_8a89601b/time31.tex <==
288s

==> assets/epm_8a89601b/time32.tex <==
300s

==> assets/epm_8a89601b/time4.tex <==
33s

==> assets/epm_8a89601b/time5.tex <==
34s

==> assets/epm_8a89601b/time6.tex <==
36s

==> assets/epm_8a89601b/time7.tex <==
36s

==> assets/epm_8a89601b/time8.tex <==
37s

==> assets/epm_8a89601b/time9.tex <==
38s

==> assets/ovo_EPM_4a37144f/options.tex <==
\item A. blue
\item B. white
\item \ANS{C. black}
\item D. red

==> assets/ovo_EPM_4a37144f/question.tex <==
what color was the phone? \texttt{[0:38]}

==> assets/ovo_EPM_4a37144f/response.tex <==
Q$\to$C \ANS{[OK]}  G$\to$C \ANS{[OK]}  I$\to$C \ANS{[OK]}

==> assets/ovo_EPM_4a37144f/time1.tex <==
0s

==> assets/ovo_EPM_4a37144f/time10.tex <==
160s

==> assets/ovo_EPM_4a37144f/time11.tex <==
200s

==> assets/ovo_EPM_4a37144f/time12.tex <==
240s

==> assets/ovo_EPM_4a37144f/time13.tex <==
280s

==> assets/ovo_EPM_4a37144f/time14.tex <==
320s

==> assets/ovo_EPM_4a37144f/time15.tex <==
360s

==> assets/ovo_EPM_4a37144f/time16.tex <==
400s

==> assets/ovo_EPM_4a37144f/time17.tex <==
440s

==> assets/ovo_EPM_4a37144f/time18.tex <==
480s

==> assets/ovo_EPM_4a37144f/time19.tex <==
520s

==> assets/ovo_EPM_4a37144f/time2.tex <==
34s

==> assets/ovo_EPM_4a37144f/time20.tex <==
560s

==> assets/ovo_EPM_4a37144f/time21.tex <==
600s

==> assets/ovo_EPM_4a37144f/time22.tex <==
640s

==> assets/ovo_EPM_4a37144f/time23.tex <==
680s

==> assets/ovo_EPM_4a37144f/time24.tex <==
720s

==> assets/ovo_EPM_4a37144f/time25.tex <==
760s

==> assets/ovo_EPM_4a37144f/time26.tex <==
800s

==> assets/ovo_EPM_4a37144f/time27.tex <==
840s

==> assets/ovo_EPM_4a37144f/time28.tex <==
880s

==> assets/ovo_EPM_4a37144f/time29.tex <==
960s

==> assets/ovo_EPM_4a37144f/time3.tex <==
35s

==> assets/ovo_EPM_4a37144f/time30.tex <==
1040s

==> assets/ovo_EPM_4a37144f/time31.tex <==
1120s

==> assets/ovo_EPM_4a37144f/time32.tex <==
1200s

==> assets/ovo_EPM_4a37144f/time4.tex <==
36s

==> assets/ovo_EPM_4a37144f/time5.tex <==
37s

==> assets/ovo_EPM_4a37144f/time6.tex <==
38s

==> assets/ovo_EPM_4a37144f/time7.tex <==
39s

==> assets/ovo_EPM_4a37144f/time8.tex <==
80s

==> assets/ovo_EPM_4a37144f/time9.tex <==
120s

==> assets/ovo_OJR_181/options.tex <==
\item A. Black Camera
\item \ANS{B. Silver round medal}
\item C. Football
\item D. Platinum round medal

==> assets/ovo_OJR_181/question.tex <==
What are these two people holding? \texttt{[15:22]}

==> assets/ovo_OJR_181/response.tex <==
Q$\to$D \WA{[X]}  G$\to$B \ANS{[OK]}  I$\to$B \ANS{[OK]}

==> assets/ovo_OJR_181/time1.tex <==
0s

==> assets/ovo_OJR_181/time10.tex <==
438s

==> assets/ovo_OJR_181/time11.tex <==
487s

==> assets/ovo_OJR_181/time12.tex <==
535s

==> assets/ovo_OJR_181/time13.tex <==
584s

==> assets/ovo_OJR_181/time14.tex <==
633s

==> assets/ovo_OJR_181/time15.tex <==
682s

==> assets/ovo_OJR_181/time16.tex <==
730s

==> assets/ovo_OJR_181/time17.tex <==
779s

==> assets/ovo_OJR_181/time18.tex <==
828s

==> assets/ovo_OJR_181/time19.tex <==
876s

==> assets/ovo_OJR_181/time2.tex <==
49s

==> assets/ovo_OJR_181/time20.tex <==
900s

==> assets/ovo_OJR_181/time21.tex <==
901s

==> assets/ovo_OJR_181/time22.tex <==
902s

==> assets/ovo_OJR_181/time23.tex <==
903s

==> assets/ovo_OJR_181/time24.tex <==
904s

==> assets/ovo_OJR_181/time25.tex <==
906s

==> assets/ovo_OJR_181/time26.tex <==
907s

==> assets/ovo_OJR_181/time27.tex <==
908s

==> assets/ovo_OJR_181/time28.tex <==
909s

==> assets/ovo_OJR_181/time29.tex <==
910s

==> assets/ovo_OJR_181/time3.tex <==
97s

==> assets/ovo_OJR_181/time30.tex <==
911s

==> assets/ovo_OJR_181/time31.tex <==
925s

==> assets/ovo_OJR_181/time32.tex <==
973s

==> assets/ovo_OJR_181/time4.tex <==
146s

==> assets/ovo_OJR_181/time5.tex <==
195s

==> assets/ovo_OJR_181/time6.tex <==
243s

==> assets/ovo_OJR_181/time7.tex <==
292s

==> assets/ovo_OJR_181/time8.tex <==
341s

==> assets/ovo_OJR_181/time9.tex <==
389s

==> assets/ovo_OJR_247/options.tex <==
\item A. The person's hand is shown with a bandage.
\item B. The person's hand is shown with a tattoo.
\item C. The person's hand is shown with a glove.
\item \ANS{D. The person's hand is shown with cuts and dirt.}

==> assets/ovo_OJR_247/question.tex <==
What is the state of the person's hand shown? \texttt{[10:40]}

==> assets/ovo_OJR_247/response.tex <==
Q$\to$D \ANS{[OK]}  G$\to$D \ANS{[OK]}  I$\to$D \ANS{[OK]}

==> assets/ovo_OJR_247/time1.tex <==
0s

==> assets/ovo_OJR_247/time10.tex <==
238s

==> assets/ovo_OJR_247/time11.tex <==
262s

==> assets/ovo_OJR_247/time12.tex <==
286s

==> assets/ovo_OJR_247/time13.tex <==
310s

==> assets/ovo_OJR_247/time14.tex <==
334s

==> assets/ovo_OJR_247/time15.tex <==
358s

==> assets/ovo_OJR_247/time16.tex <==
381s

==> assets/ovo_OJR_247/time17.tex <==
405s

==> assets/ovo_OJR_247/time18.tex <==
429s

==> assets/ovo_OJR_247/time19.tex <==
453s

==> assets/ovo_OJR_247/time2.tex <==
48s

==> assets/ovo_OJR_247/time20.tex <==
477s

==> assets/ovo_OJR_247/time21.tex <==
500s

==> assets/ovo_OJR_247/time22.tex <==
524s

==> assets/ovo_OJR_247/time23.tex <==
548s

==> assets/ovo_OJR_247/time24.tex <==
572s

==> assets/ovo_OJR_247/time25.tex <==
596s

==> assets/ovo_OJR_247/time26.tex <==
620s

==> assets/ovo_OJR_247/time27.tex <==
638s

==> assets/ovo_OJR_247/time28.tex <==
639s

==> assets/ovo_OJR_247/time29.tex <==
640s

==> assets/ovo_OJR_247/time3.tex <==
72s

==> assets/ovo_OJR_247/time30.tex <==
641s

==> assets/ovo_OJR_247/time31.tex <==
667s

==> assets/ovo_OJR_247/time32.tex <==
714s

==> assets/ovo_OJR_247/time4.tex <==
95s

==> assets/ovo_OJR_247/time5.tex <==
119s

==> assets/ovo_OJR_247/time6.tex <==
143s

==> assets/ovo_OJR_247/time7.tex <==
167s

==> assets/ovo_OJR_247/time8.tex <==
191s

==> assets/ovo_OJR_247/time9.tex <==
214s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/options.tex <==
\item A. 4080 FE, 4090 Suprim X, 4090 Matrix.
\item B. 4090 FE, 4080 Suprim X, 4090 Matrix.
\item C. 4090 FE, 4090 Suprim X, 4080 Matrix.
\item \ANS{D. 4090 FE, 4090 Suprim X, 4090 Matrix.}

==> assets/sb2_sample_119_Text-Rich_Understanding_04/question.tex <==
What graphics card models are shown on the benchmarking results right now? \texttt{[5:09]}

==> assets/sb2_sample_119_Text-Rich_Understanding_04/response.tex <==
Q$\to$D \ANS{[OK]}  G$\to$D \ANS{[OK]}  I$\to$D \ANS{[OK]}

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time1.tex <==
0s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time10.tex <==
208s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time11.tex <==
213s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time12.tex <==
218s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time13.tex <==
223s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time14.tex <==
228s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time15.tex <==
233s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time16.tex <==
237s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time17.tex <==
242s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time18.tex <==
247s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time19.tex <==
252s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time2.tex <==
26s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time20.tex <==
257s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time21.tex <==
259s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time22.tex <==
262s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time23.tex <==
285s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time24.tex <==
293s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time25.tex <==
299s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time26.tex <==
304s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time27.tex <==
310s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time28.tex <==
311s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time29.tex <==
337s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time3.tex <==
52s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time30.tex <==
349s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time31.tex <==
362s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time32.tex <==
388s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time4.tex <==
78s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time5.tex <==
104s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time6.tex <==
129s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time7.tex <==
155s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time8.tex <==
181s

==> assets/sb2_sample_119_Text-Rich_Understanding_04/time9.tex <==
207s

==> assets/sb2_sample_308_Attribute_Recognition_05/options.tex <==
\item A. Metal.
\item \ANS{B. Wood.}
\item C. Marble.
\item D. Concrete.

==> assets/sb2_sample_308_Attribute_Recognition_05/question.tex <==
What material are the stairs made of? \texttt{[8:03]}

==> assets/sb2_sample_308_Attribute_Recognition_05/response.tex <==
Q$\to$B \ANS{[OK]}  G$\to$B \ANS{[OK]}  I$\to$B \ANS{[OK]}

==> assets/sb2_sample_308_Attribute_Recognition_05/time1.tex <==
0s

==> assets/sb2_sample_308_Attribute_Recognition_05/time10.tex <==
374s

==> assets/sb2_sample_308_Attribute_Recognition_05/time11.tex <==
416s

==> assets/sb2_sample_308_Attribute_Recognition_05/time12.tex <==
457s

==> assets/sb2_sample_308_Attribute_Recognition_05/time13.tex <==
471s

==> assets/sb2_sample_308_Attribute_Recognition_05/time14.tex <==
472s

==> assets/sb2_sample_308_Attribute_Recognition_05/time15.tex <==
473s

==> assets/sb2_sample_308_Attribute_Recognition_05/time16.tex <==
474s

==> assets/sb2_sample_308_Attribute_Recognition_05/time17.tex <==
475s

==> assets/sb2_sample_308_Attribute_Recognition_05/time18.tex <==
476s

==> assets/sb2_sample_308_Attribute_Recognition_05/time19.tex <==
477s

==> assets/sb2_sample_308_Attribute_Recognition_05/time2.tex <==
42s

==> assets/sb2_sample_308_Attribute_Recognition_05/time20.tex <==
478s

==> assets/sb2_sample_308_Attribute_Recognition_05/time21.tex <==
480s

==> assets/sb2_sample_308_Attribute_Recognition_05/time22.tex <==
481s

==> assets/sb2_sample_308_Attribute_Recognition_05/time23.tex <==
482s

==> assets/sb2_sample_308_Attribute_Recognition_05/time24.tex <==
483s

==> assets/sb2_sample_308_Attribute_Recognition_05/time25.tex <==
484s

==> assets/sb2_sample_308_Attribute_Recognition_05/time26.tex <==
485s

==> assets/sb2_sample_308_Attribute_Recognition_05/time27.tex <==
486s

==> assets/sb2_sample_308_Attribute_Recognition_05/time28.tex <==
487s

==> assets/sb2_sample_308_Attribute_Recognition_05/time29.tex <==
499s

==> assets/sb2_sample_308_Attribute_Recognition_05/time3.tex <==
83s

==> assets/sb2_sample_308_Attribute_Recognition_05/time30.tex <==
540s

==> assets/sb2_sample_308_Attribute_Recognition_05/time31.tex <==
582s

==> assets/sb2_sample_308_Attribute_Recognition_05/time32.tex <==
623s

==> assets/sb2_sample_308_Attribute_Recognition_05/time4.tex <==
125s

==> assets/sb2_sample_308_Attribute_Recognition_05/time5.tex <==
166s

==> assets/sb2_sample_308_Attribute_Recognition_05/time6.tex <==
208s

==> assets/sb2_sample_308_Attribute_Recognition_05/time7.tex <==
249s

==> assets/sb2_sample_308_Attribute_Recognition_05/time8.tex <==
291s

==> assets/sb2_sample_308_Attribute_Recognition_05/time9.tex <==
332s

==> assets/sb2_sample_308_Object_Recognition_03/options.tex <==
\item A. The Green Café.
\item B. The Fun Café.
\item \ANS{C. Power Up Café.}
\item D. Stage 52 Café.

==> assets/sb2_sample_308_Object_Recognition_03/question.tex <==
What was the name of the café shown just now? \texttt{[3:04]}

==> assets/sb2_sample_308_Object_Recognition_03/response.tex <==
Q$\to$C \ANS{[OK]}  G$\to$C \ANS{[OK]}  I$\to$C \ANS{[OK]}

==> assets/sb2_sample_308_Object_Recognition_03/time1.tex <==
0s

==> assets/sb2_sample_308_Object_Recognition_03/time10.tex <==
175s

==> assets/sb2_sample_308_Object_Recognition_03/time11.tex <==
178s

==> assets/sb2_sample_308_Object_Recognition_03/time12.tex <==
180s

==> assets/sb2_sample_308_Object_Recognition_03/time13.tex <==
183s

==> assets/sb2_sample_308_Object_Recognition_03/time14.tex <==
185s

==> assets/sb2_sample_308_Object_Recognition_03/time15.tex <==
188s

==> assets/sb2_sample_308_Object_Recognition_03/time16.tex <==
190s

==> assets/sb2_sample_308_Object_Recognition_03/time17.tex <==
193s

==> assets/sb2_sample_308_Object_Recognition_03/time18.tex <==
195s

==> assets/sb2_sample_308_Object_Recognition_03/time19.tex <==
198s

==> assets/sb2_sample_308_Object_Recognition_03/time2.tex <==
42s

==> assets/sb2_sample_308_Object_Recognition_03/time20.tex <==
200s

==> assets/sb2_sample_308_Object_Recognition_03/time21.tex <==
203s

==> assets/sb2_sample_308_Object_Recognition_03/time22.tex <==
208s

==> assets/sb2_sample_308_Object_Recognition_03/time23.tex <==
249s

==> assets/sb2_sample_308_Object_Recognition_03/time24.tex <==
291s

==> assets/sb2_sample_308_Object_Recognition_03/time25.tex <==
332s

==> assets/sb2_sample_308_Object_Recognition_03/time26.tex <==
374s

==> assets/sb2_sample_308_Object_Recognition_03/time27.tex <==
416s

==> assets/sb2_sample_308_Object_Recognition_03/time28.tex <==
457s

==> assets/sb2_sample_308_Object_Recognition_03/time29.tex <==
499s

==> assets/sb2_sample_308_Object_Recognition_03/time3.tex <==
83s

==> assets/sb2_sample_308_Object_Recognition_03/time30.tex <==
540s

==> assets/sb2_sample_308_Object_Recognition_03/time31.tex <==
582s

==> assets/sb2_sample_308_Object_Recognition_03/time32.tex <==
623s

==> assets/sb2_sample_308_Object_Recognition_03/time4.tex <==
125s

==> assets/sb2_sample_308_Object_Recognition_03/time5.tex <==
165s

==> assets/sb2_sample_308_Object_Recognition_03/time6.tex <==
166s

==> assets/sb2_sample_308_Object_Recognition_03/time7.tex <==
168s

==> assets/sb2_sample_308_Object_Recognition_03/time8.tex <==
170s

==> assets/sb2_sample_308_Object_Recognition_03/time9.tex <==
173s

==> assets/sb2_sample_49_Proactive_Output_04/question.tex <==
When the cue ball touches the red ball, output "Red Touched". \texttt{[6:33]}

==> assets/sb2_sample_49_Proactive_Output_04/response.tex <==
Q: \WA{``Red Touched'' [X]}  G: \WA{``Here’s the analysis of the video and the'' [X]}  I: \WA{``Red Touched'' [X]}

==> assets/sb2_sample_49_Proactive_Output_04/time1.tex <==
0s

==> assets/sb2_sample_49_Proactive_Output_04/time10.tex <==
182s

==> assets/sb2_sample_49_Proactive_Output_04/time11.tex <==
202s

==> assets/sb2_sample_49_Proactive_Output_04/time12.tex <==
222s

==> assets/sb2_sample_49_Proactive_Output_04/time13.tex <==
242s

==> assets/sb2_sample_49_Proactive_Output_04/time14.tex <==
263s

==> assets/sb2_sample_49_Proactive_Output_04/time15.tex <==
283s

==> assets/sb2_sample_49_Proactive_Output_04/time16.tex <==
303s

==> assets/sb2_sample_49_Proactive_Output_04/time17.tex <==
323s

==> assets/sb2_sample_49_Proactive_Output_04/time18.tex <==
343s

==> assets/sb2_sample_49_Proactive_Output_04/time19.tex <==
364s

==> assets/sb2_sample_49_Proactive_Output_04/time2.tex <==
20s

==> assets/sb2_sample_49_Proactive_Output_04/time20.tex <==
384s

==> assets/sb2_sample_49_Proactive_Output_04/time21.tex <==
404s

==> assets/sb2_sample_49_Proactive_Output_04/time22.tex <==
424s

==> assets/sb2_sample_49_Proactive_Output_04/time23.tex <==
444s

==> assets/sb2_sample_49_Proactive_Output_04/time24.tex <==
465s

==> assets/sb2_sample_49_Proactive_Output_04/time25.tex <==
485s

==> assets/sb2_sample_49_Proactive_Output_04/time26.tex <==
505s

==> assets/sb2_sample_49_Proactive_Output_04/time27.tex <==
525s

==> assets/sb2_sample_49_Proactive_Output_04/time28.tex <==
545s

==> assets/sb2_sample_49_Proactive_Output_04/time29.tex <==
566s

==> assets/sb2_sample_49_Proactive_Output_04/time3.tex <==
40s

==> assets/sb2_sample_49_Proactive_Output_04/time30.tex <==
586s

==> assets/sb2_sample_49_Proactive_Output_04/time31.tex <==
606s

==> assets/sb2_sample_49_Proactive_Output_04/time32.tex <==
626s

==> assets/sb2_sample_49_Proactive_Output_04/time4.tex <==
61s

==> assets/sb2_sample_49_Proactive_Output_04/time5.tex <==
81s

==> assets/sb2_sample_49_Proactive_Output_04/time6.tex <==
101s

==> assets/sb2_sample_49_Proactive_Output_04/time7.tex <==
121s

==> assets/sb2_sample_49_Proactive_Output_04/time8.tex <==
141s

==> assets/sb2_sample_49_Proactive_Output_04/time9.tex <==
162s

==> assets/sb2_sample_49_Scene_Understanding_05/options.tex <==
\item A. A panda wearing pants meditated in front of a cherry blossom tree and said, 'Hey there,', I'm Po the Dragon Warrior.
\item B. A panda wearing pants closed its eyes and meditated in front of the cherry blossom tree, saying 'Breathe'
\item \WA{C. A panda wearing pants closed its eyes and meditated in front of the cherry blossom tree, then took a deep breath and said 'Out through the mouth' before exhaling}
\item \ANS{D. A panda wearing pants closed its eyes and meditated in front of an apple tree, then took a deep breath and said 'Out through the mouth' before exhaling}

==> assets/sb2_sample_49_Scene_Understanding_05/question.tex <==
Please describe the scene that just occurred in the video. \texttt{[7:43]}

==> assets/sb2_sample_49_Scene_Understanding_05/response.tex <==
Q$\to$A \WA{[X]}  G$\to$C \WA{[X]}  I$\to$C \WA{[X]}

==> assets/sb2_sample_49_Scene_Understanding_05/time1.tex <==
0s

==> assets/sb2_sample_49_Scene_Understanding_05/time10.tex <==
305s

==> assets/sb2_sample_49_Scene_Understanding_05/time11.tex <==
307s

==> assets/sb2_sample_49_Scene_Understanding_05/time12.tex <==
310s

==> assets/sb2_sample_49_Scene_Understanding_05/time13.tex <==
312s

==> assets/sb2_sample_49_Scene_Understanding_05/time14.tex <==
314s

==> assets/sb2_sample_49_Scene_Understanding_05/time15.tex <==
317s

==> assets/sb2_sample_49_Scene_Understanding_05/time16.tex <==
334s

==> assets/sb2_sample_49_Scene_Understanding_05/time17.tex <==
336s

==> assets/sb2_sample_49_Scene_Understanding_05/time18.tex <==
338s

==> assets/sb2_sample_49_Scene_Understanding_05/time19.tex <==
341s

==> assets/sb2_sample_49_Scene_Understanding_05/time2.tex <==
40s

==> assets/sb2_sample_49_Scene_Understanding_05/time20.tex <==
343s

==> assets/sb2_sample_49_Scene_Understanding_05/time21.tex <==
357s

==> assets/sb2_sample_49_Scene_Understanding_05/time22.tex <==
396s

==> assets/sb2_sample_49_Scene_Understanding_05/time23.tex <==
400s

==> assets/sb2_sample_49_Scene_Understanding_05/time24.tex <==
402s

==> assets/sb2_sample_49_Scene_Understanding_05/time25.tex <==
405s

==> assets/sb2_sample_49_Scene_Understanding_05/time26.tex <==
407s

==> assets/sb2_sample_49_Scene_Understanding_05/time27.tex <==
436s

==> assets/sb2_sample_49_Scene_Understanding_05/time28.tex <==
476s

==> assets/sb2_sample_49_Scene_Understanding_05/time29.tex <==
491s

==> assets/sb2_sample_49_Scene_Understanding_05/time3.tex <==
79s

==> assets/sb2_sample_49_Scene_Understanding_05/time30.tex <==
494s

==> assets/sb2_sample_49_Scene_Understanding_05/time31.tex <==
515s

==> assets/sb2_sample_49_Scene_Understanding_05/time32.tex <==
555s

==> assets/sb2_sample_49_Scene_Understanding_05/time33.tex <==
594s

==> assets/sb2_sample_49_Scene_Understanding_05/time4.tex <==
119s

==> assets/sb2_sample_49_Scene_Understanding_05/time5.tex <==
159s

==> assets/sb2_sample_49_Scene_Understanding_05/time6.tex <==
198s

==> assets/sb2_sample_49_Scene_Understanding_05/time7.tex <==
238s

==> assets/sb2_sample_49_Scene_Understanding_05/time8.tex <==
277s

==> assets/sb2_sample_49_Scene_Understanding_05/time9.tex <==
303s

==> assets/slc_ejdn67zHuEY/question.tex <==
Step localization: "make a latte"

==> assets/slc_ejdn67zHuEY/response.tex <==
GT[0]: [8.5,19.5]s IoU=0.55 ~~ GT[1]: [42.8,53.8]s IoU=0.85

==> assets/slc_ejdn67zHuEY/time1.tex <==
0s

==> assets/slc_ejdn67zHuEY/time10.tex <==
20s

==> assets/slc_ejdn67zHuEY/time11.tex <==
22s

==> assets/slc_ejdn67zHuEY/time12.tex <==
24s

==> assets/slc_ejdn67zHuEY/time13.tex <==
26s

==> assets/slc_ejdn67zHuEY/time14.tex <==
29s

==> assets/slc_ejdn67zHuEY/time15.tex <==
30s

==> assets/slc_ejdn67zHuEY/time16.tex <==
32s

==> assets/slc_ejdn67zHuEY/time17.tex <==
34s

==> assets/slc_ejdn67zHuEY/time18.tex <==
35s

==> assets/slc_ejdn67zHuEY/time19.tex <==
38s

==> assets/slc_ejdn67zHuEY/time2.tex <==
2s

==> assets/slc_ejdn67zHuEY/time20.tex <==
42s

==> assets/slc_ejdn67zHuEY/time21.tex <==
43s

==> assets/slc_ejdn67zHuEY/time22.tex <==
45s

==> assets/slc_ejdn67zHuEY/time23.tex <==
47s

==> assets/slc_ejdn67zHuEY/time24.tex <==
49s

==> assets/slc_ejdn67zHuEY/time25.tex <==
51s

==> assets/slc_ejdn67zHuEY/time26.tex <==
52s

==> assets/slc_ejdn67zHuEY/time27.tex <==
54s

==> assets/slc_ejdn67zHuEY/time28.tex <==
56s

==> assets/slc_ejdn67zHuEY/time29.tex <==
58s

==> assets/slc_ejdn67zHuEY/time3.tex <==
4s

==> assets/slc_ejdn67zHuEY/time30.tex <==
60s

==> assets/slc_ejdn67zHuEY/time31.tex <==
62s

==> assets/slc_ejdn67zHuEY/time32.tex <==
64s

==> assets/slc_ejdn67zHuEY/time4.tex <==
7s

==> assets/slc_ejdn67zHuEY/time5.tex <==
9s

==> assets/slc_ejdn67zHuEY/time6.tex <==
10s

==> assets/slc_ejdn67zHuEY/time7.tex <==
13s

==> assets/slc_ejdn67zHuEY/time8.tex <==
16s

==> assets/slc_ejdn67zHuEY/time9.tex <==
17s

==> assets/tal_video_test_0000737/question.tex <==
Find all events of: "clean and jerk"

==> assets/tal_video_test_0000737/response.tex <==
GT[0]: [20.1,43.2]s IoU=0.91 ~~ GT[1]: [80.3,90.9]s IoU=0.67 ~~ GT[2]: [116.6,134.8]s IoU=0.76

==> assets/tal_video_test_0000737/time1.tex <==
0s

==> assets/tal_video_test_0000737/time10.tex <==
43s

==> assets/tal_video_test_0000737/time11.tex <==
49s

==> assets/tal_video_test_0000737/time12.tex <==
54s

==> assets/tal_video_test_0000737/time13.tex <==
59s

==> assets/tal_video_test_0000737/time14.tex <==
64s

==> assets/tal_video_test_0000737/time15.tex <==
69s

==> assets/tal_video_test_0000737/time16.tex <==
74s

==> assets/tal_video_test_0000737/time17.tex <==
79s

==> assets/tal_video_test_0000737/time18.tex <==
80s

==> assets/tal_video_test_0000737/time19.tex <==
85s

==> assets/tal_video_test_0000737/time2.tex <==
10s

==> assets/tal_video_test_0000737/time20.tex <==
89s

==> assets/tal_video_test_0000737/time21.tex <==
90s

==> assets/tal_video_test_0000737/time22.tex <==
95s

==> assets/tal_video_test_0000737/time23.tex <==
98s

==> assets/tal_video_test_0000737/time24.tex <==
108s

==> assets/tal_video_test_0000737/time25.tex <==
114s

==> assets/tal_video_test_0000737/time26.tex <==
118s

==> assets/tal_video_test_0000737/time27.tex <==
119s

==> assets/tal_video_test_0000737/time28.tex <==
124s

==> assets/tal_video_test_0000737/time29.tex <==
128s

==> assets/tal_video_test_0000737/time3.tex <==
15s

==> assets/tal_video_test_0000737/time30.tex <==
133s

==> assets/tal_video_test_0000737/time31.tex <==
138s

==> assets/tal_video_test_0000737/time32.tex <==
147s

==> assets/tal_video_test_0000737/time4.tex <==
20s

==> assets/tal_video_test_0000737/time5.tex <==
25s

==> assets/tal_video_test_0000737/time6.tex <==
29s

==> assets/tal_video_test_0000737/time7.tex <==
34s

==> assets/tal_video_test_0000737/time8.tex <==
39s

==> assets/tal_video_test_0000737/time9.tex <==
39s

==> assets/tvg_ZjFzkhrqIZs/question.tex <==
Find event: "a shark is swimming underwater"

==> assets/tvg_ZjFzkhrqIZs/response.tex <==
GT[0]: [0.0,38.0]s IoU=0.95

==> assets/tvg_ZjFzkhrqIZs/time1.tex <==
0s

==> assets/tvg_ZjFzkhrqIZs/time10.tex <==
20s

==> assets/tvg_ZjFzkhrqIZs/time11.tex <==
23s

==> assets/tvg_ZjFzkhrqIZs/time12.tex <==
25s

==> assets/tvg_ZjFzkhrqIZs/time13.tex <==
28s

==> assets/tvg_ZjFzkhrqIZs/time14.tex <==
30s

==> assets/tvg_ZjFzkhrqIZs/time15.tex <==
33s

==> assets/tvg_ZjFzkhrqIZs/time16.tex <==
35s

==> assets/tvg_ZjFzkhrqIZs/time17.tex <==
38s

==> assets/tvg_ZjFzkhrqIZs/time18.tex <==
40s

==> assets/tvg_ZjFzkhrqIZs/time19.tex <==
45s

==> assets/tvg_ZjFzkhrqIZs/time2.tex <==
0s

==> assets/tvg_ZjFzkhrqIZs/time20.tex <==
50s

==> assets/tvg_ZjFzkhrqIZs/time21.tex <==
55s

==> assets/tvg_ZjFzkhrqIZs/time22.tex <==
60s

==> assets/tvg_ZjFzkhrqIZs/time23.tex <==
65s

==> assets/tvg_ZjFzkhrqIZs/time24.tex <==
70s

==> assets/tvg_ZjFzkhrqIZs/time25.tex <==
80s

==> assets/tvg_ZjFzkhrqIZs/time26.tex <==
90s

==> assets/tvg_ZjFzkhrqIZs/time27.tex <==
100s

==> assets/tvg_ZjFzkhrqIZs/time28.tex <==
110s

==> assets/tvg_ZjFzkhrqIZs/time29.tex <==
120s

==> assets/tvg_ZjFzkhrqIZs/time3.tex <==
3s

==> assets/tvg_ZjFzkhrqIZs/time30.tex <==
130s

==> assets/tvg_ZjFzkhrqIZs/time31.tex <==
140s

==> assets/tvg_ZjFzkhrqIZs/time32.tex <==
150s

==> assets/tvg_ZjFzkhrqIZs/time4.tex <==
5s

==> assets/tvg_ZjFzkhrqIZs/time5.tex <==
8s

==> assets/tvg_ZjFzkhrqIZs/time6.tex <==
10s

==> assets/tvg_ZjFzkhrqIZs/time7.tex <==
13s

==> assets/tvg_ZjFzkhrqIZs/time8.tex <==
15s

==> assets/tvg_ZjFzkhrqIZs/time9.tex <==
18s

==> assets/tvg_czN-9IsQXoU/question.tex <==
Find event: "a family is being recorded while having dinner"

==> assets/tvg_czN-9IsQXoU/response.tex <==
GT[0]: [98.0,118.0]s IoU=0.90

==> assets/tvg_czN-9IsQXoU/time1.tex <==
0s

==> assets/tvg_czN-9IsQXoU/time10.tex <==
70s

==> assets/tvg_czN-9IsQXoU/time11.tex <==
80s

==> assets/tvg_czN-9IsQXoU/time12.tex <==
90s

==> assets/tvg_czN-9IsQXoU/time13.tex <==
97s

==> assets/tvg_czN-9IsQXoU/time14.tex <==
98s

==> assets/tvg_czN-9IsQXoU/time15.tex <==
100s

==> assets/tvg_czN-9IsQXoU/time16.tex <==
101s

==> assets/tvg_czN-9IsQXoU/time17.tex <==
103s

==> assets/tvg_czN-9IsQXoU/time18.tex <==
104s

==> assets/tvg_czN-9IsQXoU/time19.tex <==
105s

==> assets/tvg_czN-9IsQXoU/time2.tex <==
10s

==> assets/tvg_czN-9IsQXoU/time20.tex <==
107s

==> assets/tvg_czN-9IsQXoU/time21.tex <==
108s

==> assets/tvg_czN-9IsQXoU/time22.tex <==
110s

==> assets/tvg_czN-9IsQXoU/time23.tex <==
111s

==> assets/tvg_czN-9IsQXoU/time24.tex <==
112s

==> assets/tvg_czN-9IsQXoU/time25.tex <==
114s

==> assets/tvg_czN-9IsQXoU/time26.tex <==
115s

==> assets/tvg_czN-9IsQXoU/time27.tex <==
117s

==> assets/tvg_czN-9IsQXoU/time28.tex <==
118s

==> assets/tvg_czN-9IsQXoU/time29.tex <==
120s

==> assets/tvg_czN-9IsQXoU/time3.tex <==
15s

==> assets/tvg_czN-9IsQXoU/time30.tex <==
130s

==> assets/tvg_czN-9IsQXoU/time31.tex <==
140s

==> assets/tvg_czN-9IsQXoU/time32.tex <==
150s

==> assets/tvg_czN-9IsQXoU/time4.tex <==
20s

==> assets/tvg_czN-9IsQXoU/time5.tex <==
25s

==> assets/tvg_czN-9IsQXoU/time6.tex <==
30s

==> assets/tvg_czN-9IsQXoU/time7.tex <==
40s

==> assets/tvg_czN-9IsQXoU/time8.tex <==
50s

==> assets/tvg_czN-9IsQXoU/time9.tex <==
60s

==> sec/0_abstract.tex <==
\begin{abstract}
Recent progress in video large language models (Video-LLMs) has enabled strong offline reasoning over long and complex videos. However, real-world deployments increasingly require streaming perception and proactive interaction, where video frames arrive online and the system must decide not only what to respond, but also when to respond. In this work, we revisit proactive activation in streaming video as a structured sequence modeling problem, motivated by the observation that temporal transitions in streaming video naturally form span-structured activation patterns. To capture this span-level structure, we model activation signals jointly over a sliding temporal window and update them iteratively as new frames arrive. We propose \textit{STRIDE} (Structured Temporal Refinement with Iterative DEnoising), which employs a lightweight masked diffusion module at the activation interface to jointly predict and progressively refine activation signals across the window. Extensive experiments on diverse streaming benchmarks and downstream models demonstrate that \textit{STRIDE} shows more reliable and temporally coherent proactive responses, significantly improving ``when-to-speak'' decision quality in online streaming scenarios.
\keywords{Proactive Video Streaming \and Activation Modeling \and Masked Diffusion Model}
\end{abstract}

